Costless: Optimizing Cost of Serverless Computing through Function Fusion and Placement

Serverless computing has recently experienced significant adoption by several applications, especially Internet of Things (IoT) applications. In serverless computing, rather than deploying and managing dedicated virtual machines, users are able to deploy individual functions, and pay only for the time that their code is actually executing. However, since serverless platforms are relatively new, they have a completely different pricing model that depends on the memory, duration, and the number of executions of a sequence/workflow of functions. In this paper we present an algorithm that optimizes the price of serverless applications in AWS Lambda. We first describe the factors affecting price of serverless applications which include: (1) fusing a sequence of functions, (2) splitting functions across edge and cloud resources, and (3) allocating the memory for each function. We then present an efficient algorithm to explore different function fusion-placement solutions and find the solution that optimizes the application's price while keeping the latency under a certain threshold. Our results on image processing workflows show that the algorithm can find solutions optimizing the price by more than 35%-57% with only 5%-15% increase in latency. We also show that our algorithm can find non-trivial memory configurations that reduce both latency and price.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> _intro.tex <==
\section{Introduction}

The continued growth of Internet of Things (IoT) applications requires the ability to extract insights from massive amounts of data streams observed at real-time. The data could be collected from multiple input sources such as: (1) surveillance cameras for traffic monitoring and intrusion detection, (2) wearable cameras and medical devices for healthcare, (3) sensors deployed on bridges and buildings in smart cities.

%Machine learning (ML) techniques have become quite useful in processing large amounts of incoming data from IoT systems, to perform complex tasks such as vision and speech processing. Typically ML models are trained in the cloud and deployed on edge~\cite{edge} devices for real-time predictions/inference. However these edge devices have limited computational capability. And sending the data streams to powerful remote servers for model inference may not be feasible, given the latency and bandwidth requirements for transferring complex data such as video streams. So a key challenge is to automatically decide how to partition such inference models among edge and cloud compute resources, in order to minimize the overall completion time of inference task.  

Due to limited computational capability of IoT devices that collect such data, the conventional approach of performing analytics on data streams is to send them to the cloud and leverage its powerful resources to execute analytics remotely. However, given the tremendous amount of data transfer often required (e.g., when video data is collected), the latency and bandwidth requirements become very high. This calls for an alternative paradigm in which ML models are trained in the cloud and then deployed on the edge~\cite{edge} for near real-time inference (i.e. execution of pre-trained ML model operations). 

ML models consist of a large number of dependent operations modeled as dataflow graphs~\cite{tensorflow}. Each operation describes computation on the incoming data such as matrix multiplication or convolution. A key challenge is to automatically decide how to partition operations by assigning them to edge and cloud resources, in order to minimize the overall completion time of the entire graph of operations. Our work addresses this problem and makes the following contributions:

% Due to the limited computational capability of devices that collect such data, the conventional approach of performing analytics on data streams is to send the stream to a centralized data center and leverage its powerful and seemingly abundant resources to execute the analytics remotely. However, given the tremendous amount of data transfer required by video data as an example, the latency and bandwidth requirements become significantly high. These issues become particularly significant in IoT systems that include smartphones, cameras, smart sensors, etc. And it becomes a key driver for a machine learning (ML) paradigm in which models are trained in the public cloud and then deployed in the edge~\cite{edge} for near real-time predictions/inference.
% Since these models perform complex calculations on large amounts of real-time data (for tasks such as vision and speech processing), a key challenge is to automatically decide how to partition such graphs among an edge and cloud compute resources in order to minimize the overall completion time of DAG of operations. 

%ML models consist of large number of dependent operations modeled as dataflow graphs~\cite{tensorflow}. Each operation describes some computation on the incoming data such as matrix multiplication or convolution. In this paper, we make the following contributions to the operator placement problem of assigning each operator to an edge or cloud resource:
\begin{enumerate}
\item We propose a general model for scheduling of dataflow graphs that operate on a data stream of observations/inputs. The model considers computation, communication and queuing delays, and captures pipeline parallelism for estimating execution time. Such pipelining arises due to multiple inputs being processed concurrently by different operators in the graph.
% \item We propose an operator placement algorithm that addresses diverse requirements of IoT workloads such as: (1) data coming as a continuous stream of observations that have queuing delays, (2) heterogeneous and geo-distributed compute and network resources.
% \item We propose a model for the scheduling/execution of IoT workloads that captures: (1) data coming as a continuous stream of observations that have queuing delays, (2), (2) heterogeneous and geo-distributed compute and network resources.

\item We draw an analogy between operator placement problem and Matrix Chain Ordering Problem (MCOP) which allows us to design a dynamic programming algorithm to solve the operator placement in $O(m \cdot (L!) \cdot L)$ complexity, where $m$ is the number of operators and $L$ is the number of resources. %(e.g., typically one edge and one cloud) ).
\end{enumerate}

Other approaches based on reinforcement learning (RL) techniques~\cite{RL} have been proposed to solve the operator placement problem and shown to be effective for static resource configurations. However, our approach targets dynamic environments in which connectivity between edge devices change rapidly. %and the algorithm have to account for such changes in the environment. 











%Moreover, if the cloud infrastructure belongs to a public cloud provider that charges for consumed compute, network, and storage resources, this approach of cloud-centric analytics becomes prohibitively expensive. 



==> _proposed.tex <==
% \section{Operator Placement}\label{sec:placement}
\section{Problem Definition}

Given a dataflow graph $G$ with a set of vertices $G_o =\{o_{1},o_{2},o_{3},...,o_{m}\}$, each vertex in the graph corresponds to one operator. Each operator processes $n$ inputs, where an input is one unit of data defined by the application (e.g., tuple, video frame). Links between vertices correspond to dataflow dependency between operators. If $G$ has a link from operator $o_{1}$ to operator $o_{2}$, then each input $n_i$ has to be processed first by $o_{1}$ before it is transmitted to $o_{2}$. Let $R$ be a resource graph $R$ with a set of vertices $R_v=\{r_1,r_2,r_3,..,r_L\}$. Each resource represents an edge device (such as smartphone), intermediate server, or the cloud. 

Each operator $o_{i}$ has an execution cost when placed on any of the $p$ resources in $R_v$. The execution cost for $o_{i}$ is represented as $(t_{o_{i,1}}, ...t_{o_{i,L}})$ and the intermediate data is represented as $d_{i}$. Each resource $r_k$ is connected to some other resource $r_l$ with connection speed $s_{kl}$. The operator placement problem is defined as the mapping $M$ of operators to resources such that the completion time of the last operator $o_{m}$ is minimized. 
We define $M$ as $\{ M: G_o \rightarrow R_v \implies M(o_{i}) = \{ r_{l}\ \in R_v \} \}$


%The operator placement problem is defined as the mapping $M$ of operators to resources such that the completion time of the last operator $o_{m}$  is minimized. We define $M$ as $M = (m_{o_{1}},..,m_{o_{t}})$ such that $m_{o_{i}} \in R_v$ represent the resource where operator $o_{i}$ is placed.

%The operator placement problem is defined as minimizing the function $f$, which denotes the completion time and resource consumption cost of all inputs. 
%in the current placement interval (see Eq.~\ref{obj-fun}) 
%This is done by finding a mapping $M$ from operators to resources such that
%$\{ M: G \rightarrow R \implies M(o_{i,k}) = M_{i,k} = \{ r_{l}\ \in\  r_{l} \in R \} \}$, where $M_{i,k} = r_{l}$ implies that operator $o_{i,k}$ is executed in compute resource $r_{l}$

%finding a mapping $M$ from operators to resources such that
%$\{ M: G \rightarrow R \implies M(o_{i,k}) = M_{i,k} = \{ r_{l}\ \in\  r_{l} \in R \} \}$, where $M_{i,k} = r_{l}$ implies that operator $o_{i,k}$ is executed in compute resource $r_{l}$

%The overall execution time can then be formulated as:
%$E = t_{n,k_n} - t_{0,0})$, such that $t_{n,k_n}$ is the completion time of the last task in the last task graph, while $t(1,0)$ is the time step just before task 1 of the first task graph start execution. The completion time $t_{n,k_n}$ is a function of the completion time of all the previous tasks $t_{i,j}$ and the completion time for the fist task $t_{1,1}$ is a function of its execution cost $e_{i,j}$ and its communication cost. The problem of task placement can be defined as:
%$$M^*= \min_{M}\ E$$


\section{Proposed Approach}\label{sec:placement}
The key idea in our approach is to leverage the fact that each operator in a dataflow graph $G$ has to process $n$ inputs. Hence, two dependent operators can be concurrently processing inputs in a pipeline fashion. For example, the first input that was processed by operator $o_{1}$, can now be processed by $o_{2}$ while the second input is being processed in parallel by $o_{1}$. This pipelining behavior is only applicable if there are enough resources to execute multiple operators in parallel. For simplicity, we assume that each resource has one thread or unit of computation, however, the method can be generalized to resources with multiple threads or containers. The pipelining behavior can reduce the computation time through parallelism however, it introduces a transmission latency when two dependent operators are placed on different resources. Hence, the problem becomes how to choose which operators to run in parallel in order to reduce the overall computation and communication time. Consider the following example:

\subsection{Illustrative Example}
Assume that we have a sequence of three operators $o_1$, $o_2$, $o_3$ and two different resources: (1) an edge device $E$, (2) a cloud VM $C$. The possible options to place our operators between the two resources are shown in Figure~\ref{fig:matrixbracket}. Each line in the figure shows a different possibility for operator placement. The subscript $(1,E)$ means that operator 1 is placed on device $E$ and operators inside parentheses show that they are executed in a pipelined manner. 
% 	$$(o_{1,E}), (o_{2,E}) ,(o_{3,E})$$
%     $$(o_{1,E}), (o_{2,E} , o_{3,C})$$
%     $$(o_{1,E}, o_{2,C}) , (o_{3,E})$$
%     $$(o_{1,E}, o_{2,C}) , (o_{3,C})$$
%     $$(o_{1,C}, o_{2,E}) , (o_{3,E}) $$
%     $$(o_{1,C}, o_{2,E}) , (o_{3,C}) $$
%     $$(o_{1,C}), (o_{2,C}, o_{3,E}) $$
%     $$(o_{1,C}), (o_{2,C}), (o_{3,C}) $$

\begin{figure}
% \centering
\begin{minipage}{.15\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{MatrixBracketingPlacement.PNG}
  \captionof{figure}{Different operator\\ placements}
  \label{fig:matrixbracket}
\end{minipage}%
\begin{minipage}{.35\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{PlacementGraph_SysMl.PNG}
  \captionof{figure}{Corresponding placement graph. The difference between dashed and solid edges, along with other graph details are discussed in section~\ref{sec:solution}}
  \label{fig:placementgraph}
\end{minipage}
\end{figure}

Using the representation in Figure~\ref{fig:matrixbracket} for the placement of operators on resources helps us draw an analogy between operator placement and the matrix chain ordering problem (MCOP)~\cite{mcop}. Recall that in MCOP, the problem is to find the most efficient way to multiply a given sequence of matrices together. There exists a dynamic programming algorithm for solving MCOP in polynomial time. Section~\ref{sec:solution} describes how this analogy can be similarly used to reduce the complexity of solving operator placement problem from exponential to polynomial time in the number of operators. 

\subsection{Solution} \label{sec:solution}

In order to represent the solutions in Figure~\ref{fig:matrixbracket}, we construct the {\it placement graph} shown in Figure~\ref{fig:placementgraph}. The dashed edges in placement graph show connections between operators running in parallel (i.e., the ones collocated inside the parentheses), however the solid edges are between operators at the boundaries of two sets of parentheses. The dashed edges have resource cost because going from one dashed edge to another means that you are executing the next operator on a new thread or a new server which results in increased overall resource consumption. The solid edges are the ones that have computation and communication costs (see Figure~\ref{fig:placementgraph}). The intuition for reduction in placement problem complexity is that the paths 
$[(o_{1,E}, o_{2,C}), (o_{3,C})]$ and $[(o_{1,C}, o_{2,E}) , (o_{3,C})]$ have a common solid edge going from $(o_{3,C})$ to the $END$ node. There are however two separate edges going to $(o_{3,C})$, which help differentiate between the two paths, one edge has the cost of path $(o_{1,E}, o_{2,C})$ and the other has the cost of path $(o_{1,C}, o_{2,E})$.

We note that the shortest path between start and end nodes is the solution of the operator placement problem. For example, if the shortest path is $[(o_{1,E}, o_{2,C}) , (o_{3,C})]$, then the placement will be $o_1$ on device $E$ while $o_2$ and $o_3$ are on the device $C$.

{\bf Limitations}: Our approach has an implicit assumption that when operators $(o_{1,E}, o_{2,C})$ are executed concurrently, they will fully utilize available resources and that's why $(o_{3,C})$ has to wait for device $C$ resources to be free. However, this may not be the case; in the future, we plan to explore the optimal number of inputs that can be processed concurrently by $o_2$ to fully utilize device $C$.
\subsection{Cost Calculation:}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{pipeline.png}
\caption{Execution of tasks $o_{1,E}$ and $o_{2,C}$ in parallel in different devices.}
\label{fig:pipelining}
\end{figure}

We describe how to calculate the overall computation and communication cost of operators inside the parentheses in figure~\ref{fig:placementgraph}, such as cost of $(o_{1,E}, o_{2,C})$ in the path $[(o_{1,E}, o_{2,C}), (o_{3,C})]$. Figure~\ref{fig:pipelining} illustrates how $o_{1,E}$ and $ o_{2,C}$ operators are processing inputs in a pipeline fashion. Let's assume we have 3 video frames and two operators $o_1$ and $o_2$ that process each video frame in sequence. The first operator is placed on device $E$ and the second on device $C$. Frame 1 is first provided to operator $o_1$ and then transmitted to device $C$ where operator $o_2$ can be applied to it, while operator $o_1$ is being applied to frame 2 concurrently. The overall cost is the time for the last video frame to finish execution at $o_2$. The cost of the $n^{th}$ video frame is given by:

%\begin{equation} \label{eq3}
%\begin{split}
$Cost( (o_{1,E}, o_{2,C}) ) = (n-1) t_{o_{1,E}} + t_{o_{1,E}}  +  tr\{E \rightarrow C\}  + t_{o_{2,C}}$ \\
%\end{split}
%\end{equation}
where $tr\{E \rightarrow C\}$ is the cost of transmitting data from $E$ to $C$.\\

%We note that the previous equation is applicable when $o_2$ is dependent on $o_1$, however if $o_1$ and $o_2$ are operators in parallel paths in a DAG, then the cost is given by 
%\begin{equation} \label{eq3}
%\begin{split}

%\hspace{2cm}$Cost( (o_{1,E}, o_{2,C}) ) = max(n\cdot t_{o_{1,E}}, n\cdot t_{o_{2,C}})$
%\end{split}
%\end{equation}


%Equation~\ref{eq3} is derived based on the assumption that $t_{o_{1,E}} > t_{o_{2,C}}$ as shown in Figure~\ref{fig:pipelining}. The general formula for $Cost (o_{1,E}, o_{2,C})$ is:

%\begin{equation} \label{eq3}
%\begin{split}
%Cost( (o_{1,E}, o_{2,C}) ) = (n-1) max(t_{o_{1,E}}, t_{o_{2,C}}, tr\{o_{1,E},o_{2,C}\} ) \\ + t_{o_{1,E}} + t_{o_{2,C}} + tr\{o_{1,E},o_{2,C}\}
%\end{split}
%\end{equation}
\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{TaskBased_1.png}
  \captionof{figure}{Scalability comparison between our proposed approach and brute force approach.}
  %Brute force search time is cutoff for more than 5 operators because it was very large.}
  %in the time to search for the best placement
  \label{fig:complexity}
\end{figure}
\section{Evaluation}

We evaluate the scalability of our approach in terms of time to search for a placement that minimizes the operators' execution time. We compare our solution with a brute force (BF) approach that searches over all possible operator placements. BF searches over $O(r^m)$ solutions, where $m$ is the number of operators and $r$ is the number of resources. We vary the number of operators in the input graph. Both approaches have the same placement result for instances in which BF finished in reasonable time (up to 5 operators). Moreover, we show the scalability of our approach in Figure~\ref{fig:complexity}. Results show that the proposed algorithm linearly scales in the number of operators as opposed to an exponential increase in the running time of BF approach.
%, and b. This confirms the scalability of our approach which has a complexity of $O(mr^2)$.






